Backdoor Mitigation by Correcting the Distribution of Neural Activations

Backdoor (Trojan) attacks are an important type of adversarial exploit against deep neural networks (DNNs), wherein a test instance is (mis)classified to the attacker's target class whenever the attacker's backdoor trigger is present. In this paper, we reveal and analyze an important property of backdoor attacks: a successful attack causes an alteration in the distribution of internal layer activations for backdoor-trigger instances, compared to that for clean instances. Even more importantly, we find that instances with the backdoor trigger will be correctly classified to their original source classes if this distribution alteration is corrected. Based on our observations, we propose an efficient and effective method that achieves post-training backdoor mitigation by correcting the distribution alteration using reverse-engineered triggers. Notably, our method does not change any trainable parameters of the DNN, but achieves generally better mitigation performance than existing methods that do require intensive DNN parameter tuning. It also efficiently detects test instances with the trigger, which may help to catch adversarial entities in the act of exploiting the backdoor.

==> ref.tex <==
\bibitem[{Bengio, Y. et~al.(2007) Bengio, Y. \& LeCun, Y.}]{Bengio+chapter2007}
Bengio, Y. \& LeCun, Y. (2007).
\newblock Scaling Learning Algorithms Towards AI. 
\newblock {\em Large Scale Kernel Machines}. 

\bibitem[{Hinton, G. et~al.(2006) Hinton, G., Osindero, S. \& Teh, Y.}]{Hinton06}
Hinton, G., Osindero, S. \& Teh, Y. (2006).
\newblock A Fast Learning Algorithm for Deep Belief Nets. 
\newblock {\em Neural Computation}. \textbf{18} pp. 1527-1554 

\bibitem[{Goodfellow, I. et~al.(2016) Goodfellow, I., Bengio, Y., Courville, A. \& Bengio, Y.}]{goodfellow2016deep}
Goodfellow, I., Bengio, Y., Courville, A. \& Bengio, Y. (2016).
\newblock Deep learning. 
\newblock {\em MIT Press}

\bibitem[{Li, Y. et~al.(2022) Li, Y., Jiang, Y., Li, Z. \& Xia, S.}]{BAsurvey}
Li, Y., Jiang, Y., Li, Z. \& Xia, S. (2022).
\newblock Backdoor Learning: A Survey. 
\newblock {\em IEEE Transactions On Neural Networks And Learning Systems}. pp. 1-18 

\bibitem[{Ilyas, A. et~al.(2019) Ilyas, A., Santurkar, S., Tsipras, D., Engstrom, L., Tran, B. \& Madry, A.}]{Ilyas_NIPS_2019}
Ilyas, A., Santurkar, S., Tsipras, D., Engstrom, L., Tran, B. \& Madry, A. (2019).
\newblock Adversarial Examples Are Not Bugs, They Are Features. 
\newblock {\em NeurIPS}. 

\bibitem[{Frankle, J. et~al.(2021) Frankle, J., Schwab, D. \& Morcos, A.}]{FrankleSM21}
Frankle, J., Schwab, D. \& Morcos, A. (2021).
\newblock Training BatchNorm and Only BatchNorm: On the Expressive Power of Random Features in CNNs. 
\newblock {\em ICLR}. 

\bibitem[{Li, X. et~al.(2022) Li, X., Xiang, Z., Miller, D. \& Kesidis, G.}]{InFlight}
Li, X., Xiang, Z., Miller, D. \& Kesidis, G. (2022).
\newblock Test-Time Detection of Backdoor Triggers for Poisoned Deep Neural Networks. 
\newblock {\em ICASSP}. 

\bibitem[{Benz, P. et~al.(2021) Benz, P., Zhang, C., Karjauv, A. \& Kweon, I.}]{Benz_2021_WACV}
Benz, P., Zhang, C., Karjauv, A. \& Kweon, I. (2021).
\newblock Revisiting Batch Normalization for Improving Corruption Robustness. 
\newblock {\em WACV}. 

\bibitem[{Zhao, Z. et~al.(2022) Zhao, Z., Chen, X., Xuan, Y., Dong, Y., Wang, D. \& Liang, K. }]{Zhao_2022_CVPR}
Zhao, Z., Chen, X., Xuan, Y., Dong, Y., Wang, D. \& Liang, K. (2022).
\newblock DEFEAT: Deep Hidden Feature Backdoor Attacks by Imperceptible Perturbation and Latent Representation Constraints. 
\newblock {\em CVPR}. 

\bibitem[{Qi, X. et~al.(2022) Qi, X., Xie, T., Pan, R., Zhu, J., Yang, Y. \& Bu, K.}]{Qi_2022_CVPR}
Qi, X., Xie, T., Pan, R., Zhu, J., Yang, Y. \& Bu, K. (2022).
\newblock Towards Practical Deployment-Stage Backdoor Attack on Deep Neural Networks. 
\newblock {\em CVPR}. 

\bibitem[{Xie, C.et~al.(2020) Xie, C., Huang, K., Chen, P. \& Li, B.}]{Xie2020DBA}
Xie, C., Huang, K., Chen, P. \& Li, B. (2020).
\newblock DBA: Distributed Backdoor Attacks against Federated Learning. 
\newblock {\em ICLR}. 

\bibitem[{Wang, Z. et~al.(2022) Wang, Z., Zhai, J. \& Ma, S.}]{Wang_2022_CVPR}
Wang, Z., Zhai, J. \& Ma, S. (2022).
\newblock BppAttack: Stealthy and Efficient Trojan Attacks Against Deep Neural Networks via Image Quantization and Contrastive Adversarial Learning. 
\newblock {\em CVPR}. 

\bibitem[{Yao, Y. et~al.(2019) Yao, Y., Li, H., Zheng, H. \& Zhao, B.}]{Yao_2019_CCS}
Yao, Y., Li, H., Zheng, H. \& Zhao, B. (2019).
\newblock Latent Backdoor Attacks on Deep Neural Networks. 
\newblock {\em Proceedings Of The 2019 ACM SIGSAC Conference On Computer And Communications Security}. 

\bibitem[{Wang, L. et~al.(2021) Wang, L., Javed, Z., Wu, X., Guo, W., Xing, X. \& Song, D.}]{Wang_2021_IJCAI}
Wang, L., Javed, Z., Wu, X., Guo, W., Xing, X. \& Song, D. (2021).
\newblock BACKDOORL: Backdoor Attack against Competitive Reinforcement Learning. 
\newblock {\em IJCAI}. 

\bibitem[{Xiang, Z. et~al.(2019) Xiang, Z., Miller, D. \& Kesidis, G.}]{CI}
Xiang, Z., Miller, D. \& Kesidis, G. (2019).
\newblock A benchmark study of backdoor data poisoning defenses for deep neural network classifiers and a novel defense. 
\newblock {\em MLSP}. 

\bibitem[{Zhang, Z. et~al.(2022) Zhang, Z., Lyu, L., Wang, W., Sun, L. \& Sun, X.}]{zhang2022how}
Zhang, Z., Lyu, L., Wang, W., Sun, L. \& Sun, X. (2022).
\newblock How to Inject Backdoors with Better Consistency: Logit Anchoring on Clean Data. 
\newblock {\em ICLR}. 

\bibitem[{Schneider, S. et~al.(2020) Schneider, S., Rusak, E., Eck, L., Bringmann, O., Brendel, W. \& Bethge, M.}]{SchneiderRE0BB20}
Schneider, S., Rusak, E., Eck, L., Bringmann, O., Brendel, W. \& Bethge, M. (2020).
\newblock Improving robustness against common corruptions by covariate shift adaptation. 
\newblock {\em NeurIPS}. 

\bibitem[{Santurkar, S.et~al.(2018) Santurkar, S., Tsipras, D., Ilyas, A. \& Madry, A.}]{SanturkarTIM18}
Santurkar, S., Tsipras, D., Ilyas, A. \& Madry, A. (2018).
\newblock How Does Batch Normalization Help Optimization?. 
\newblock {\em NeurIPS}. 

\bibitem[{Lubana, E.et~al.(2021) Lubana, E., Dick, R. \& Tanaka, H.}]{lubana2021beyond}
Lubana, E., Dick, R. \& Tanaka, H. (2021).
\newblock Beyond BatchNorm: Towards a Unified Understanding of Normalization in Deep Learning. 
\newblock {\em NeurIPS}. 

\bibitem[{Ioffe, S. et~al.(2015) Ioffe, S. \& Szegedy, C.}]{IoffeS15}
Ioffe, S. \& Szegedy, C. (2015).
\newblock Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift. 
\newblock {\em ICML}. 

\bibitem[{Li, X. et~al.(2021) Li, X., Kesidis, G., Miller, D. \& Lucic, V.}]{LKML21}
Li, X., Kesidis, G., Miller, D. \& Lucic, V. (2021).
\newblock Backdoor Attack and Defense for Deep Regression. 
\newblock {\em ArXiv}. 2109.02381

\bibitem[{Krizhevsky, A.(2009)}]{cifar10}
Krizhevsky, A. (2009).
\newblock Learning multiple layers of features from tiny images. 
\newblock \url{http://www.cs.toronto.edu/ kriz/learning-features-2009-TR.pdf}

\bibitem[{Wang, B. et~al.(2019) Wang, B., Yao, Y., Shan, S., Li, H., Viswanath, B., Zheng, H. \& Zhao, B.}]{NC}
Wang, B., Yao, Y., Shan, S., Li, H., Viswanath, B., Zheng, H. \& Zhao, B. (2019).
\newblock Neural Cleanse: Identifying and Mitigating Backdoor Attacks in Neural Networks. 
\newblock {\em 2019 IEEE Symposium On Security And Privacy}. 

\bibitem[{Gao, Y. et~al.(2019) Gao, Y., Xu, C., Wang, D., Chen, S., Ranasinghe, D. \& Nepal, S.}]{STRIP}
Gao, Y., Xu, C., Wang, D., Chen, S., Ranasinghe, D. \& Nepal, S. (2019).
\newblock STRIP: a defence against trojan attacks on deep neural networks. 
\newblock {\em ACSAC}. 

\bibitem[{Liu, Y. et~al.(2018) Liu, Y., Ma, S., Aafer, Y., Lee, W., Zhai, J., Wang, W. \& Zhang, X.}]{Trojan}
Liu, Y., Ma, S., Aafer, Y., Lee, W., Zhai, J., Wang, W. \& Zhang, X. (2018).
\newblock Trojaning Attack on Neural Networks. 
\newblock {\em NDSS}. 

\bibitem[{Gu, T. et~al.(2019) Gu, T., Liu, K., Dolan-Gavitt, B. \& Garg, S.}]{BadNets}
Gu, T., Liu, K., Dolan-Gavitt, B. \& Garg, S. (2019).
\newblock BadNets: Evaluating Backdooring Attacks on Deep Neural Networks. 
\newblock {\em IEEE Access}. 

\bibitem[{Chen, X. et~al.(2017) Chen, X., Liu, C., Li, B., Lu, K. \& Song, D.}]{Targeted-Backdoor}
Chen, X., Liu, C., Li, B., Lu, K. \& Song, D. (2017).
\newblock Targeted Backdoor Attacks on Deep Learning Systems Using Data Poisoning. 
\newblock {\em ArXiv}. 1712.05526

\bibitem[{Dong, Y. et~al.(2021) Dong, Y., Yang, X., Deng, Z., Pang, T., Xiao, Z., Su, H. \& Zhu, J.}]{B3D}
Dong, Y., Yang, X., Deng, Z., Pang, T., Xiao, Z., Su, H. \& Zhu, J. (2021).
\newblock Black-box Detection of Backdoor Attacks with Limited Information and Data. 
\newblock {\em ICCV}. 

\bibitem[{Doan, K.et~al.(2021) Doan, K., Lao, Y. \& Li, P.}]{WB}
Doan, K., Lao, Y. \& Li, P. (2021).
\newblock Backdoor Attack with Imperceptible Input and Latent Modification. 
\newblock {\em NeurIPS}. 

\bibitem[{Hampel, F.(1974)}]{MAD}
Hampel, F. (1974).
\newblock The influence curve and its role in robust estimation. 
\newblock {\em Journal Of The American Statistical Association}. 

\bibitem[{Chou, E. et~al.(2020) Chou, E., Tramèr, F. \& Pellegrino, G.}]{SentiNet}
Chou, E., Tramèr, F. \& Pellegrino, G. (2020).
\newblock SentiNet: Detecting Localized Universal Attacks Against Deep Learning Systems. 
\newblock {\em 2020 IEEE Security And Privacy Workshops}. 

\bibitem[{Xiang, Z. et~al.(2020) Xiang, Z., Miller, D. \& Kesidis, G.}]{TNNLS}
Xiang, Z., Miller, D. \& Kesidis, G. (2020).
\newblock Detection of Backdoors in Trained Classifiers Without Access to the Training Set. 
\newblock {\em IEEE Transactions On Neural Networks And Learning Systems}. 

\bibitem[{He, K. et~al.(2016) He, K., Zhang, X., Ren, S. \& Sun, J.}]{ResNet}
He, K., Zhang, X., Ren, S. \& Sun, J. (2016).
\newblock Deep Residual Learning for Image Recognition. 
\newblock {\em CVPR}. 

\bibitem[{Howard, A. et~al.(2017) Howard, A., Zhu, M., Chen, B., Kalenichenko, D., Wang, W., Weyand, T., Andreetto, M. \& Adam, H.}]{MobileNet}
Howard, A., Zhu, M., Chen, B., Kalenichenko, D., Wang, W., Weyand, T., Andreetto, M. \& Adam, H. (2017).
\newblock MobileNets: Efficient Convolutional Neural Networks for Mobile Vision Applications. 
\newblock {\em ArXiv}. 1704.04861

\bibitem[{Kingma, D. et~al.(2015) Kingma, D. \& Ba, J.}]{Adam}
Kingma, D. \& Ba, J. (2015).
\newblock Adam: A Method for Stochastic Optimization. 
\newblock {\em ICLR}. 

\bibitem[{Wang, S. et~al.(2020) Wang, S., Nepal, S., Rudolph, C., Grobler, M., Chen, S. \& Chen, T.}]{BackdoorTransferLearning}
Wang, S., Nepal, S., Rudolph, C., Grobler, M., Chen, S. \& Chen, T. (2020).
\newblock Backdoor Attacks against Transfer Learning with Pre-trained Deep Learning Models. 
\newblock {\em IEEE Transactions On Services Computing}. 

\bibitem[{Yao, Y. et~al.(2019) Yao, Y., Li, H., Zheng, H. \& Zhao, B.}]{DBLP:conf/ccs/YaoLZZ19}
Yao, Y., Li, H., Zheng, H. \& Zhao, B. (2019).
\newblock Latent Backdoor Attacks on Deep Neural Networks. 
\newblock {\em Proceedings Of The 2019 ACM SIGSAC Conference On Computer And Communications Security}. 

\bibitem[{Li, S. et~al.(2019) Li, S., Zhao, B., Yu, J., Xue, M., Kaafar, D. \& Zhu, H.}]{DBLP:journals/corr/abs-1909-02742}
Li, S., Zhao, B., Yu, J., Xue, M., Kaafar, D. \& Zhu, H. (2019).
\newblock Invisible Backdoor Attacks Against Deep Neural Networks. 
\newblock {\em ArXiv}. 1909.02742

\bibitem[{Saha, A. et~al.(2020) Saha, A., Subramanya, A. \& Pirsiavash, H.}]{HiddenTrigger}
Saha, A., Subramanya, A. \& Pirsiavash, H. (2020).
\newblock Hidden Trigger Backdoor Attacks. 
\newblock {\em AAAI}. 

\bibitem[{Miller, D. et~al.(2019) Miller, D., Wang, Y. \& Kesidis, G.}]{TTE}
Miller, D., Wang, Y. \& Kesidis, G. (2019).
\newblock When Not to Classify: Anomaly Detection of Attacks (ADA) on DNN Classifiers at Test Time. 
\newblock {\em Neural Comput.}. 

\bibitem[{Chen, X. et~al.(2020) Chen, X., Salem, A., Backes, M., Ma, S. \& Zhang, Y.}]{DBLP:journals/corr/abs-2006-01043}
Chen, X., Salem, A., Backes, M., Ma, S. \& Zhang, Y. (2020).
\newblock BadNL: Backdoor Attacks Against NLP Models. 
\newblock {\em ArXiv}. 2006.01043 

\bibitem[{Dai, J. et~al.(2019) Dai, J., Chen, C. \& Li, Y.}]{8836465}
Dai, J., Chen, C. \& Li, Y. (2019).
\newblock A Backdoor Attack Against LSTM-Based Text Classification Systems. 
\newblock {\em IEEE Access}. 

\bibitem[{Liu, K. et~al.(2018) Liu, K., Dolan-Gavitt, B. \& Garg, S.}]{Fine-Pruning}
Liu, K., Dolan-Gavitt, B. \& Garg, S. (2018).
\newblock Fine-Pruning: Defending Against Backdooring Attacks on Deep Neural Networks. 
\newblock {\em RAID}. 

\bibitem[{Guo, W. et~al.(2019) Guo, W., Wang, L., Xing, X., Du, M. \& Song, D.}]{TABOR}
Guo, W., Wang, L., Xing, X., Du, M. \& Song, D. (2019)
\newblock TABOR: A Highly Accurate Approach to Inspecting and Restoring Trojan Backdoors in AI Systems. 
\newblock {\em ArXiv}. 1908.01763

\bibitem[{Xiang, Z. et~al.(2020) Xiang, Z., Miller, D. \& Kesidis, G.}]{DBLP:conf/icassp/XiangMK20}
Xiang, Z., Miller, D. \& Kesidis, G. (2020).
\newblock Revealing Backdoors, Post-Training, in DNN Classifiers via Novel Inference on Optimized Perturbations Inducing Group Misclassification. 
\newblock {\em ICASSP}. 

\bibitem[{Shen, Y. et~al.(2019) Shen, Y. \& Sanghavi, S.}]{trim_loss}
Shen, Y. \& Sanghavi, S. (2019).
\newblock Learning with Bad Training Data via Iterative Trimmed Loss Minimization. 
\newblock {\em ICML}. pp. 5739-5748 

\bibitem[{Madry, A. et~al.(2018) Madry, A., Makelov, A., Schmidt, L., Tsipras, D. \& Vladu, A.}]{PGD}
Madry, A., Makelov, A., Schmidt, L., Tsipras, D. \& Vladu, A. (2018).
\newblock Towards Deep Learning Models Resistant to Adversarial Attacks. 
\newblock {\em ICLR}. 

\bibitem[{Doan, B. et~al.(2020) Doan, B., Abbasnejad, E. \& Ranasinghe, D.}]{Februus}
Doan, B., Abbasnejad, E. \& Ranasinghe, D. (2020).
\newblock Februus: Input Purification Defense Against Trojan Attacks on Deep Neural Network Systems. 
\newblock {\em Annual Computer Security Applications Conference}. pp. 897-912 

\bibitem[{Kolouri, S. et~al.(2020) Kolouri, S., Saha, A., Pirsiavash, H. \& Hoffmann, H.}]{meta_sup}
Kolouri, S., Saha, A., Pirsiavash, H. \& Hoffmann, H. (2020).
\newblock Universal Litmus Patterns: Revealing Backdoor Attacks in CNNs. 
\newblock {\em CVPR}. pp. 298-307 

\bibitem[{Xu, X. et~al.(2021) Xu, X., Wang, Q., Li, H., Borisov, N., Gunter, C. \& Li, B.}]{meta_unsup}
Xu, X., Wang, Q., Li, H., Borisov, N., Gunter, C. \& Li, B. (2021).
\newblock Detecting AI Trojans Using Meta Neural Analysis. 
\newblock {\em Proc. IEEE Symposium On Security And Privacy}. 

\bibitem[{Wang, R. et~al.(2020) Wang, R., Zhang, G., Liu, S., Chen, P., Xiong, J. \& Wang, M.}]{DataLimited}
Wang, R., Zhang, G., Liu, S., Chen, P., Xiong, J. \& Wang, M. (2020).
\newblock Practical Detection of Trojan Neural Networks: Data-Limited and Data-Free Cases. 
\newblock {\em ECCV}. 

\bibitem[{Du, M. et~al.(2020) Du, M., Jia, R. \& Song, D.}]{Differential_Privacy}
Du, M., Jia, R. \& Song, D. (2020).
\newblock Robust Anomaly Detection and Backdoor Attack Detection Via Differential Privacy. 
\newblock {\em ICLR}. 

\bibitem[{Li, Y. et~al.(2021) Li, Y., Lyu, X., Koren, N., Lyu, L., Li, B. \& Ma, X.}]{li2021anti}
Li, Y., Lyu, X., Koren, N., Lyu, L., Li, B. \& Ma, X. (2021).
\newblock Anti-Backdoor Learning: Training Clean Models on Poisoned Data. 
\newblock {\em NeurIPS}. 

\bibitem[{Xiang, Z. et~al.(2019) Xiang, Z., Miller, D. \& Kesidis, G.}]{MLSP}
Xiang, Z., Miller, D. \& Kesidis, G. (2019).
\newblock A Benchmark Study Of Backdoor Data Poisoning Defenses For Deep Neural Network Classifiers And A Novel Defense. 
\newblock {\em MLSP}. 

\bibitem[{Liu, Y. et~al.(2019) Liu, Y., Lee, W., Tao, G., Ma, S., Aafer, Y. \& Zhang, X.}]{ABS}
Liu, Y., Lee, W., Tao, G., Ma, S., Aafer, Y. \& Zhang, X. (2019).
\newblock ABS: Scanning Neural Networks for Back-Doors by Artificial Brain Stimulation. 
\newblock {\em Proceedings Of The 2019 ACM SIGSAC Conference On Computer And Communications Security}. pp. 1265-1282 

\bibitem[{Chen, H. et~al.(2019) Chen, H., Fu, C., Zhao, J. \& Koushanfar, F.}]{DeepInspect}
Chen, H., Fu, C., Zhao, J. \& Koushanfar, F. (2019).
\newblock DeepInspect: A Black-box Trojan Detection and Mitigation Framework for Deep Neural Networks. 
\newblock {\em IJCAI}. pp. 4658-4664 

\bibitem[{Dong, Y. et~al.(2021) Dong, Y., Yang, X., Deng, Z., Pang, T., Xiao, Z., Su, H. \& Zhu, J.}]{NC_blackbox}
Dong, Y., Yang, X., Deng, Z., Pang, T., Xiao, Z., Su, H. \& Zhu, J. (2021).
\newblock Black-box Detection of Backdoor Attacks with Limited Information and Data.
\newblock {\em ICCV}.  

\bibitem[{Miller, D. et~al.(2020) Miller, D., Xiang, Z. \& Kesidis, G.}]{Proceedings}
Miller, D., Xiang, Z. \& Kesidis, G. (2020).
\newblock Adversarial Learning Targeting Deep Neural Network Classification: A Comprehensive Review of Defenses Against Attacks. 
\newblock {\em Proc. IEEE}. 

\bibitem[{Tran, B. et~al.(2018) Tran, B., Li, J. \& Madry, A.}]{SS}
Tran, B., Li, J. \& Madry, A. (2018).
\newblock Spectral Signatures in Backdoor Attacks. 
\newblock {\em NeurIPS}. 

\bibitem[{Chen, B. et~al.(2019) Chen, B., Carvalho, W., Baracaldo, N., Ludwig, H., Edwards, B., Lee, T., Molloy, I. \& Srivastava, B.}]{AC}
Chen, B., Carvalho, W., Baracaldo, N., Ludwig, H., Edwards, B., Lee, T., Molloy, I. \& Srivastava, B. (2019).
\newblock Detecting Backdoor Attacks on Deep Neural Networks by Activation Clustering. 
\newblock {\em AAAI}. 

\bibitem[{Simonyan, K. et~al.(2015) Simonyan, K. \& Zisserman, A.}]{VGG}
Simonyan, K. \& Zisserman, A. (2015).
\newblock Very Deep Convolutional Networks for Large-Scale Image Recognition. 
\newblock {\em ICLR}. 

\bibitem[{Lecun, Y. et~al.(1998) Lecun, Y., Bottou, L., Bengio, Y. \& Haffner, P.}]{LeNet}
Lecun, Y., Bottou, L., Bengio, Y. \& Haffner, P. (1998).
\newblock Gradient-based learning applied to document recognition. 
\newblock {\em Proceedings Of The IEEE}. 

\bibitem[{Kumar, N. et~al.(2009) Kumar, N., Berg, A., Belhumeur, P. \& Nayar, S.}]{PubFig}
Kumar, N., Berg, A., Belhumeur, P. \& Nayar, S. (2009).
\newblock Attribute and Simile Classifiers for Face Verification. 
\newblock {\em ICCV}. 

\bibitem[{Deng, L.(2012)}]{MNIST}
Deng, L. (2012).
\newblock The mnist database of handwritten digit images for machine learning research. 
\newblock {\em IEEE Signal Processing Magazine}. 

\bibitem[{Xiao, H. et~al.(2017) Xiao, H., Rasul, K. \& Vollgraf, R.}]{FMNIST}
Xiao, H., Rasul, K. \& Vollgraf, R. (2017).
\newblock Fashion-MNIST: a Novel Image Dataset for Benchmarking Machine Learning Algorithms.  
\newblock {\em ArXiv}. 1708.07747

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem[{Xiang, Z. et~al.(2021) Xiang, Z., Miller, D., Chen, S., Li, X. \& Kesidis, G.}]{ZhenICCV}
Xiang, Z., Miller, D., Chen, S., Li, X. \& Kesidis, G. (2021).
\newblock A Backdoor Attack against 3D Point Cloud Classifiers. 
\newblock {\em ICCV}. 

\bibitem[{Xiang, Z. et~al.(2022) Xiang, Z., Miller, D., Chen, S., Li, X. \& Kesidis, G.}]{XiangMCLK22}
Xiang, Z., Miller, D., Chen, S., Li, X. \& Kesidis, G. (2022).
\newblock Detecting Backdoor Attacks against Point Cloud Classifiers. 
\newblock {\em ICASSP}. 

\bibitem[{Li, Y. et~al.(2017) Li, Y., Wang, N., Shi, J., Liu, J. \& Hou, X.}]{AdaBN}
Li, Y., Wang, N., Shi, J., Liu, J. \& Hou, X. (2017).
\newblock Revisiting Batch Normalization For Practical Domain Adaptation. 
\newblock {\em ICLR}. 

\bibitem[{Ioffe, S. et~al.(2015) Ioffe, S. \& Szegedy, C.}]{BN}
Ioffe, S. \& Szegedy, C. (2015).
\newblock Batch Normalization: Accelerating Deep Network Training by Reducing Internal Covariate Shift. 
\newblock {\em ICML}. 

\bibitem[{Zeng, Y. et~al.(2022) Zeng, Y., Chen, S., Park, W., Mao, Z., Jin, M. \& Jia, R.}]{hypergrad}
Zeng, Y., Chen, S., Park, W., Mao, Z., Jin, M. \& Jia, R. (2022).
\newblock Adversarial Unlearning of Backdoors via Implicit Hypergradient. 
\newblock {\em ICLR}. 

\bibitem[{Ali, S. et~al.(1966) Ali, S. \& Silvey, S.}]{Ali1966AGC}
Ali, S. \& Silvey, S. (1966).
\newblock A General Class of Coefficients of Divergence of One Distribution from Another. 
\newblock {\em Journal Of The Royal Statistical Society Series B-methodological}. \textbf{28} pp. 131-142 

\bibitem[{Li, Y. et~al.(2021) Li, Y., Lyu, X., Koren, N., Lyu, L., Li, B. \& Ma, X.}]{NAD}
Li, Y., Lyu, X., Koren, N., Lyu, L., Li, B. \& Ma, X. (2021).
\newblock Neural Attention Distillation: Erasing Backdoor Triggers from Deep Neural Networks. 
\newblock {\em ICLR}. 

\bibitem[{Nguyen, T. et~al.(2021) Nguyen, T. \& Tran, A.}]{WaNet}
Nguyen, T. \& Tran, A. (2021).
\newblock WaNet - Imperceptible Warping-based Backdoor Attack. 
\newblock {\em ICLR}. 

\bibitem[{Li, S. et~al.(2021) Li, S., Xue, M., Zhao, B., Zhu, H. \& Zhang, X.}]{invisible}
Li, S., Xue, M., Zhao, B., Zhu, H. \& Zhang, X. (2021).
\newblock Invisible Backdoor Attacks on Deep Neural Networks Via Steganography and Regularization. 
\newblock {\em IEEE Transactions On Dependable And Secure Computing}. \textbf{18}, 2088-2105 

\bibitem[{Huang, K. et~al.(2022) Huang, K., Li, Y., Wu, B., Qin, Z. \& Ren, K.}]{huang2022backdoor}
Huang, K., Li, Y., Wu, B., Qin, Z. \& Ren, K. (2022).
\newblock Backdoor Defense via Decoupling the Training Process. 
\newblock {\em ICLR}. 

\bibitem[{Wu, D. et~al.(2021) Wu, D. \& Wang, Y.}]{ANP}
Wu, D. \& Wang, Y. (2021).
\newblock Adversarial Neuron Pruning Purifies Backdoored Deep Models. 
\newblock {\em NeurIPS}. 

\bibitem[{Zheng, R. et~al.(2022) Zheng, R., Tang, R., Li, J. \& Liu, L.}]{CLP}
Zheng, R., Tang, R., Li, J. \& Liu, L. (2022).
\newblock Data-free Backdoor Removal based on Channel Lipschitzness. 
\newblock {\em ECCV}. 

\bibitem[{Guan, J. et~al.(2022) Guan, J., Tu, Z., He, R. \& Tao, D.}]{ShapPruning}
Guan, J., Tu, Z., He, R. \& Tao, D. (2022).
\newblock Few-shot Backdoor Defense Using Shapley Estimation. 
\newblock {\em CVPR}. 

\bibitem[{Xia, J. et~al.(2022) Xia, J., Wang, T., Ding, J., Wei, X. \& Chen, M.}]{ARGD}
Xia, J., Wang, T., Ding, J., Wei, X. \& Chen, M. (2022).
\newblock Eliminating Backdoor Triggers for Deep Neural Networks Using Attention Relation Graph Distillation. 
\newblock {\em IJCAI}. 

\bibitem[{Barni, M. et~al.(2019) Barni, M., Kallas, K. \& Tondi, B.}]{SIG}
Barni, M., Kallas, K. \& Tondi, B. (2019).
\newblock A New Backdoor Attack in {CNNS} by Training Set Corruption Without Label Poisoning.
\newblock {\em ICIP}

\bibitem[{Wang, H. et~al.(2022) Wang, H., Xiang, Z., Miller, D. \& Kesidis, G.}]{UniBD}
Wang, H., Xiang, Z., Miller, D. \& Kesidis, G. (2022).
\newblock Universal Post-Training Backdoor Detection. 
\newblock {\em ArXiv}. \textbf{2205.069} 

\bibitem[{Bai, J. et~al.(2022) Bai, J., Gao, K., Gong, D., Xia, S., Li, Z. \& Liu, W.}]{Bai_2022_ECCV}
Bai, J., Gao, K., Gong, D., Xia, S., Li, Z. \& Liu, W. (2022).
\newblock Hardly Perceptible Trojan Attack against Neural Networks with Bit Flips. 
\newblock {\em ECCV}. 

\bibitem[{Liu, Y. et~al.(2022) Liu, Y., Shen, G., Tao, G., Wang, Z., Ma, S. \& Zhang, X.}]{Liu_2022_CVPR}
Liu, Y., Shen, G., Tao, G., Wang, Z., Ma, S. \& Zhang, X. (2022).
\newblock Complex Backdoor Detection by Symmetric Feature Differencing. 
\newblock {\em CVPR}. 

\bibitem[{Tao, G. et~al.(2022) Tao, G., Shen, G., Liu, Y., An, S., Xu, Q., Ma, S., Li, P. \& Zhang, X.}]{Tao_2022_CVPR}
Tao, G., Shen, G., Liu, Y., An, S., Xu, Q., Ma, S., Li, P. \& Zhang, X. (2022).
\newblock Better Trigger Inversion Optimization in Backdoor Scanning. 
\newblock {\em CVPR}. 

\bibitem[{Houben, S. et~al.(2013) Houben, S., Stallkamp, J., Salmen, J., Schlipsing, M. \& Igel, C.}]{GTSRB}
Houben, S., Stallkamp, J., Salmen, J., Schlipsing, M. \& Igel, C. (2013).
\newblock Detection of Traffic Signs in Real-World Images: The German Traffic Sign Detection Benchmark. 
\newblock {\em International Joint Conference On Neural Networks}. 

\bibitem[{Howard, J. (2020)}]{imagewang}
Howard, J. (2020). 
\newblock ImageNette. 
\newblock https://github.com/fastai/imagenette/

\bibitem[{Le, Y. et~al.(2015) Le, Y. \& Yang, X.}]{TinyImageNet}
Le, Y. \& Yang, X. (2015).
\newblock Tiny ImageNet Visual Recognition Challenge. 
\newblock https://tiny-imagenet.herokuapp.

\bibitem[{Russakovsky, O. et~al.(2015) Russakovsky, O., Deng, J., Su, H., Krause, J., Satheesh, S., Ma, S., Huang, Z., Karpathy, A., Khosla, A., Bernstein, M., Berg, A. \& Fei-Fei, L.}]{ImageNet}
Russakovsky, O., Deng, J., Su, H., Krause, J., Satheesh, S., Ma, S., Huang, Z., Karpathy, A., Khosla, A., Bernstein, M., Berg, A. \& Fei-Fei, L. (2015).
\newblock ImageNet Large Scale Visual Recognition Challenge. 
\newblock {\em Int. J. Comput. Vis.}. \textbf{115}, 211-252 
